C2C: Cough to COVID-19 Detection in BHI 2023 Data Challenge

This report describes our submission to BHI 2023 Data Competition: Sensor challenge. Our Audio Alchemists team designed an acoustic-based COVID-19 diagnosis system, Cough to COVID-19 (C2C), and won the 1st place in the challenge. C2C involves three key contributions: pre-processing of input signals, cough-related representation extraction leveraging Wav2vec2.0, and data augmentation. Through experimental findings, we demonstrate C2C's promising potential to enhance the diagnostic accuracy of COVID-19 via cough signals. Our proposed model achieves a ROC-AUC value of 0.7810 in the context of COVID-19 diagnosis. The implementation details and the python code can be found in the following link: https://github.com/Woo-jin-Chung/BHI_2023_challenge_Audio_Alchemists

==> 6_Acknowledgements.tex <==
\section*{ACKNOWLEDGMENT}
\label{sec:acknowledgements}
This work was supported by the project `Alchemist Brain to X (B2X) Project' through
the Ministry of Trade, Industry and Energy (MOTIE), South Korea, under Grant 20012355 and NTIS 1415181023. 
